Imitater: An Efficient Shared Mempool Protocol with Application to Byzantine Fault Tolerance

Byzantine Fault Tolerant (BFT) consensus, a cornerstone of blockchain technology, has seen significant advancements. While existing BFT protocols ensure security guarantees, they often suffer from efficiency challenges, particularly under conditions of network instability or malicious exploitation of system mechanisms. We propose a novel Shared Mempool (SMP) protocol, named Imitater, which can be seamlessly integrated into BFT protocols. By chaining microblocks and applying coding techniques, Imitater efficiently achieves \emph{totality} and \emph{availability}. Furthermore, a BFT protocol augmented with Imitater ensures \emph{order preservation} of client transactions while mitigating the risks of \emph{over-distribution} and \emph{unbalanced workload}. In the experiment, we integrate Imitater into the HotStuff protocol, resulting in Imitater-HS. The performance of Imitater-HS is validated in a system with up to 256 nodes. Experimental results demonstrate the efficiency of our approach: Imitater-HS achieves higher throughput and lower latency in the presence of faulty nodes compared to Stratus-HS, the state-of-the-art protocol. Notably, the throughput improvement increases with the number of faulty nodes.

==> disscussion.tex <==
%\section{Discussion}
%\label{Sec:disscussion}
%\textbf{Unbalanced work load.}在Section~\ref{subsec:timingOfMbDiss}我们讨论了带宽波动的场景，但是可能存在一些其他的模型。在实际部署场景中，客户端可能会就近，或者向更信任的节点发送自己的tx请求，因此，各共识节点所承受的负担实际上可能是不一致的，某些节点可能会承受过多的负担而其他节点则可能会闲置。Stratus的方法是让过载的节点将分发microblock的任务外包给其他闲置节点，但这样无疑会增大延迟，而且最坏情况需要请求很多次才能完成分发的任务。但是在Imitater-BFT中，则可以无缝地适应这个场景，只需要允许闲置、无分发任务的节点可以重复报告最高AC。过载的节点可以很轻易的将分发的任务平摊到其他节点身上。


%讨论bft协议部分只是我们给出的一个样例，实施山可以使用其他性质的bft，比如Efficient-HS等从而获得一些其他的property。

% \textbf{Proof choice to replace merkle tree.}
% 在Section~\ref{sec:SMP_detail}中我们使用merkle证明来证明不同的编码块和来自相同的microblock，节点对默克尔根进行签名，表示对对应的microblock锁进行的ack回复。但是实际上对于证明的选择并不单一， \cite{alhaddad2021succinct}提出的ECP对编码块进行证明，还有利用stark对编码块作证明的工作\cite{civit2023every}，这些工作尝试证明编码块和原始数据块是对应的，但是在bft的场景中，不需要这么强的约束。
% proof是为了帮助实现EC correctness和EC consistency，即证明不同的编码块组合所解码出的结果是一致的。我们的obvervation是对编码块的标识符做证明足矣。于是除了merkle之外一个可行替代方案是使用RSA累加器，与默克尔树相比，RSA Accumulator有着更小的通信开销和更大的计算开销，且需要trusted setup。
% 直觉上计算对一个microblock计算RSA证明需要O(n)次群幂操作，导致不使用，但是介于这个proof是可以在microblock打包完成后、分发前进行计算，从而抵消计算时间带来的影响，从而或许是一个不错的选择。上述的证明选择可以说是一个trade-off，或许需要协议的部署者去选择自己需要的证明方式。我们将在后续的工作中讨论最佳的proof 选择。
% \begin{table}[!h]
%     \centering
%     \begin{tabular}{c|ccc}
%         \hline
%          & Comm & Comp & Trust setup\\ \hline
%         RSA Accumulator &  &  & \\ \hline
%         Merkle Proof &  &  & \\ \hline
%     \end{tabular}
%     \caption{Caption}
%     \label{tab:my_label}
% \end{table}

% In Section~\ref{sec:SMP_detail}, we utilize Merkle proofs to verify that different chunks originate from the same microblock, with nodes signing the Merkle root as an acknowledgment of the corresponding microblock. However, the choice of proof is not limited to this approach. For instance, ECP, as proposed in \cite{alhaddad2021succinct}, provides proofs for chunks, and there are also efforts utilizing STARKs to prove the correspondence between chunks and the original data block \cite{civit2023every}. These approaches aim to establish a strong link between chunks and the original data, but such stringent constraints are unnecessary in a BFT context.

% The primary purpose of proofs in this setting is to ensure EC correctness and EC consistency, i.e., to verify that the results decoded from different combinations of chunks are consistent. Our observation is that proving the identifiers of chunks suffices. Therefore, besides Merkle trees, another viable alternative is using RSA accumulators. Compared to Merkle trees, RSA accumulators offer lower communication overhead but come with higher computational costs and require a trusted setup.

% Intuitively, computing RSA proofs for a microblock requires \( O(n) \) group exponentiations, which might initially seem prohibitive. However, since these proofs can be computed after the microblock is packaged and before it is distributed, the impact of computation time could be mitigated, making RSA accumulators a potentially attractive option. The choice of proof method represents a trade-off, and it may be up to the protocol deployers to decide which proof mechanism best suits their needs. We will explore the optimal proof selection in future work.


% \textbf{Trade-off?} RSA不抗量子，而且RSA需要trusted setup来保证group order不为人所知，其通信开销为n个域元素。
% merkle有着更大的证明size,以及更小的计算。 

% 直观上O(n)数量的群幂运算或许会是一笔很大的开销，导致这个工具并不实用。事实上，在某种程度上RSA的方案或许更好，因为这个proof的计算实际上是可以提前进行的，由于只是对content进行编码与证明，在一个leader-robin的系统中，节点可以提前计算这些proof，并在当选leader的时候直接使用。

% 上述的证明选择可以说是一个trade-off，或许需要协议的部署者去选择自己需要的证明方式，只需要替换CreatProof和VerifyProof即可。

